Norm-induced Cuts: Outer Approximation for Lipschitzian Constraint Functions

In this paper, we consider a finite-dimensional optimization problem minimizing a continuous objective on a compact domain subject to a multi-dimensional constraint function. For the latter, we assume the availability of a global Lipschitz constant. In recent literature, methods based on non-convex outer approximation are proposed for tackling one-dimensional equality constraints that are Lipschitz with respect to the maximum norm. To the best of our knowledge, however, there does not exist a non-convex outer approximation method for a general problem class. We introduce a meta-level solution framework to solve such problems and tackle the underlying theoretical foundations. Considering the feasible domain without the constraint function as manageable, our method relaxes the multidimensional constraint and iteratively refines the feasible region by means of norm-induced cuts, relying on an oracle for the resulting subproblems. We show the method's correctness and investigate the problem complexity. In order to account for discussions about functionality, limits, and extensions, we present computational examples including illustrations.

==> data-1d-berthold.tex <==
iteration {cuts added} {objective value}
0 0 1.0
1 1 1.721026232851378
2 2 2.192121990881836
3 3 2.893034446128991
4 4 3.348112578878293
5 5 3.474792904506367
6 6 3.8545492195228386
7 7 3.884104818053844
8 9 3.978319046595733
9 10 4.126305711235031
10 11 4.595457088296176
11 12 4.768787799662279
12 13 4.930644471937146
13 14 5.020948441115491
14 15 5.043897114474993
15 16 5.072613832405578
16 17 5.17844819272777
17 18 5.449838442906704
18 19 5.565463042473442
19 21 5.677327253581279
20 22 5.700024824949103
21 23 5.729455646789681
22 24 5.856175439025452
23 26 5.973143593031824
24 27 5.985030373548986
25 28 6.041859059094464
26 29 6.103704884727627
27 30 6.107293325864833
28 31 6.135987199481898
29 32 6.171186643905825
30 33 6.185354965600474
31 34 6.197038415464589
32 35 6.255103602089653
33 37 6.302787212491815
34 38 6.325554734728323
35 39 6.3526011329166385
36 40 6.393012105437379
37 41 6.40109682557773
38 42 6.452800415753426
39 43 6.499449516152049
40 44 6.5021809302405185
41 45 6.50873629367033
42 46 6.515599457430866
43 47 6.523299491314827
44 48 6.52902317024395
45 49 6.554445531798883
46 50 6.569120817528072
47 51 6.582121359763393
48 52 6.5845957932736905
49 53 6.593620398567843
50 55 6.595704569816889
51 56 6.597064951574868
52 57 6.604819242533022
53 58 6.620950333433063
54 59 6.623620421288479
55 60 6.6263593432835055
56 61 6.629207107159354
57 62 6.63154465962071
58 63 6.637483894002742
59 64 6.640552500352266
60 65 6.640677383304225
61 66 6.649991353552232
62 67 6.655601420670745
63 68 6.65696360924935
64 69 6.658982530165611
65 70 6.663799494794466
66 71 6.666681947412471
67 72 6.6706079125093485
68 73 6.674261794976928
69 74 6.675838949304755
70 75 6.677969510011348
71 76 6.687041204112462
72 77 6.689403991445962
73 78 6.690888265590235
74 79 6.692168691831728
75 80 6.6926917068813525
76 81 6.694815558538772
77 82 6.6968027599844255
78 83 6.69707129838066
79 84 6.698935923332559
80 85 6.70238624337825
81 86 6.7026024080382545
82 87 6.705102831519582
83 88 6.70792393584029
84 89 6.70892647153016
85 90 6.711206868171944
86 91 6.712534676798951
87 92 6.712890673717133
88 93 6.715059898053183
89 94 6.716314027565634
90 95 6.718504271259405
91 96 6.718824245623057
92 97 6.719589924370727
93 98 6.720670282941173
94 99 6.7210827511679225
95 100 6.721127539812412
96 101 6.72162817300793
97 102 6.722017014729971
98 103 6.723773215673617
99 104 6.724721824094179


==> data-1d-berthold_manip.tex <==
iteration {cuts added} {objective value}
0 0 1.0
1 2 1.5887154558316776
2 4 1.925119455099562
3 6 2.457921175873643
4 8 2.782126826972997
5 10 2.8486841989210276
6 12 3.2894848838259105
7 14 3.326037376954445
8 16 3.6425041644509353
9 18 3.672627576993645
10 20 3.768791112734622
11 22 3.835764845021131
12 24 4.077848966932625
13 26 4.233335491919424
14 28 4.391670337292903
15 30 4.398606379241306
16 32 4.688451952231144
17 34 4.706299019132114
18 36 4.822609275203111
19 38 4.961308512667766
20 40 4.986945701067801
21 42 5.1723443938224305
22 44 5.178097281938885
23 46 5.185484424541517
24 48 5.259593673788972
25 50 5.337419701167212
26 52 5.347506444598919
27 54 5.418993972931277
28 56 5.521359846989162
29 58 5.565120493486307
30 60 5.633317928088449
31 62 5.736800935506014
32 64 5.742459061178441
33 66 5.773460002295932
34 68 5.796820335723202
35 70 5.832150083791629
36 72 5.852488546075859
37 74 5.85976628247148
38 76 5.929941092032356
39 78 6.027428585581887
40 80 6.04670123539519
41 82 6.049936711450837
42 84 6.083015981512454
43 86 6.094875697365153
44 88 6.1095655961010005
45 90 6.110519720292697
46 92 6.21026372913104
47 94 6.214391563917288
48 96 6.214859538912486
49 98 6.230923042110252
50 100 6.247377724780975
51 102 6.287370624879752
52 104 6.318458760583075
53 106 6.327757014413828
54 108 6.333347220256723
55 110 6.342292817314805
56 112 6.396986106171221
57 114 6.399300759429413
58 116 6.414906060868812
59 118 6.428949369249047
60 120 6.430628585630094
61 122 6.431610958281174
62 124 6.454352866823948
63 126 6.465212944169882
64 128 6.48200633763914
65 130 6.487583751381279
66 132 6.494509748590842
67 134 6.497162644293104
68 136 6.501408906987983
69 138 6.510838006789871
70 140 6.511137746966656
71 142 6.531659316581835
72 144 6.536794786948923
73 146 6.545092497590996
74 148 6.560330504121973
75 150 6.560631249035257
76 152 6.567944467563522
77 154 6.568785284654713
78 156 6.571525760340804
79 158 6.571628105885911
80 160 6.572364036266487
81 162 6.579948646309276
82 164 6.589472928387819
83 166 6.594573869374129
84 168 6.597644982404528
85 170 6.597774486029328
86 172 6.599002868540602
87 174 6.601901436645817
88 176 6.6106936083938015
89 178 6.619990192817244
90 180 6.620625922052852
91 182 6.622992454321698
92 184 6.6239196837009375
93 186 6.630188281804879
94 188 6.6315797844219135
95 190 6.639484973278344
96 192 6.63979220147966
97 194 6.641779957418952
98 196 6.6420582173206215
99 198 6.6425486999865235


==> data-2d-berthold.tex <==
iteration {cuts added} {objective value}
0 0 1.0
1 1 1.319811683712214
2 2 1.567737629773792
3 3 1.750091398119234
4 4 1.969248587472293
5 5 2.137879879796139
6 6 2.1789636001575863
7 7 2.272994479154234
8 8 2.4016913411938603
9 9 2.465661338630072
10 10 2.559040613332534
11 11 2.745724198289486
12 12 2.772453372917524
13 13 2.8621399359569617
14 14 2.947671030834687
15 15 3.0304866235997
16 16 3.135787985733852
17 17 3.147707929489984
18 18 3.203972792861191
19 19 3.227922404709626
20 20 3.297286715104662
21 21 3.382615973284548
22 22 3.425774813182115
23 23 3.477344080102845
24 24 3.48432540787086
25 25 3.541326459809661
26 26 3.6823147953829
27 27 3.728856588334838
28 28 3.742160986934899
29 29 3.7525329384118864
30 30 3.8030081619312206
31 31 3.818320328348005
32 32 3.908050575192776
33 33 3.931849591306747
34 34 3.99519288143186
35 35 4.05500103212926
36 36 4.092016960992192
37 37 4.129284805342798
38 38 4.178422786135974
39 39 4.186367104066871
40 40 4.229831419377952
41 41 4.237957244486086
42 42 4.333758589509875
43 43 4.342458620870583
44 44 4.358144276194171
45 45 4.36659118659305
46 46 4.3777187410899785
47 47 4.389688801436096
48 48 4.399449173566516
49 49 4.418170013136172
50 50 4.508964617440904
51 51 4.514712044119565
52 52 4.5741254674700915
53 53 4.602891820448531
54 54 4.604825676464081
55 55 4.712430167124198
56 56 4.714558493216038
57 57 4.737142304245237
58 58 4.737373615809188
59 59 4.756942908158763
60 60 4.770637695175941
61 61 4.859305151843644
62 62 4.884832314102115
63 63 4.893925656781272
64 64 4.918501848399589
65 65 4.920501869256736
66 66 4.941772648315227
67 67 4.953850137599636
68 68 4.989406882299956
69 69 5.040451568151692
70 70 5.042116459490459
71 71 5.065464383259608
72 72 5.079023336979896
73 73 5.103245290922008
74 74 5.105487890330462
75 75 5.144244526733846
76 76 5.150772993931645
77 77 5.156711907197212
78 78 5.1795545239339695
79 79 5.2031095064728845
80 80 5.203631367615049
81 81 5.244212144995788
82 82 5.266837773503101
83 83 5.282566451633974
84 84 5.301331868285734
85 85 5.306220868411916
86 86 5.315529610782881
87 87 5.32148423679435
88 88 5.335032521925592
89 89 5.343776990547309
90 90 5.344357668561621
91 91 5.371410639693024
92 92 5.403150609238887
93 93 5.411003294347174
94 94 5.43390627485633
95 95 5.464407697800669
96 96 5.474622953397091
97 97 5.477802473970615
98 98 5.489913780045436
99 99 5.508936354681294


==> data-2d-berthold_manip.tex <==
iteration {cuts added} {objective value}
0 0 1.0
1 1 1.721026232851088
2 2 2.192121990881332
3 3 2.893034446128751
4 4 3.3481203130057713
5 5 3.474792898278246
6 6 3.8545531643224673
7 7 3.8841045628351383
8 8 3.978319112761397
9 9 4.126304326637601
10 10 4.59545729234206
11 11 4.7687827530500115
12 12 4.930643862656492
13 13 5.021329877474942
14 14 5.043897225854585
15 15 5.07261756479229
16 16 5.178484976725602
17 17 5.449429364702644
18 18 5.565876982780257
19 19 5.677327498116556
20 20 5.699972200934039
21 21 5.7294486790417745
22 22 5.856172401345279
23 23 5.972984783739982
24 24 5.984987290119968
25 25 6.041486717489391
26 26 6.10370768108613
27 27 6.107293743221327
28 28 6.13598740114249
29 29 6.171323455999839
30 30 6.185256915157938
31 31 6.197037478020226
32 32 6.255957498232519
33 33 6.302818486022728
34 34 6.325555318459636
35 35 6.352039313477432
36 36 6.392890954868698
37 37 6.401340869188998
38 38 6.452832736925318
39 39 6.499203097962657
40 40 6.50226629499169
41 41 6.50870567374099
42 42 6.515528628597863
43 43 6.523416035900492
44 44 6.528841132943651
45 45 6.554453466429357
46 46 6.569121800192157
47 47 6.582014701389039
48 48 6.5845538473170215
49 49 6.59362504885218
50 50 6.595590456155794
51 51 6.597017596097245
52 52 6.604912976352493
53 53 6.620582821709376
54 54 6.62368217947014
55 55 6.626526490512618
56 56 6.629120343268574
57 57 6.631542548813702
58 58 6.637477362516482
59 59 6.640411196089254
60 60 6.640682767909982
61 61 6.649972382987457
62 62 6.655675397926317
63 63 6.656960803913326
64 64 6.6589595642017585
65 65 6.66364541409574
66 66 6.666685573342132
67 67 6.670620876484399
68 68 6.6742582690596475
69 69 6.675892164809325
70 70 6.678037055073725
71 71 6.68727703567934
72 72 6.689441160280182
73 73 6.690694191251956
74 74 6.69212681385933
75 75 6.692848812735039
76 76 6.694591686309784
77 77 6.697036825430493
78 78 6.697113358188286
79 79 6.699137909716505
80 80 6.702495471631601
81 81 6.702624227357745
82 82 6.705206355156486
83 83 6.707693156738583
84 84 6.708986399306605
85 85 6.711458835665297
86 86 6.712856841274452
87 87 6.713036247065816
88 88 6.715150999109316
89 89 6.716528297323887
90 90 6.71853735876158
91 91 6.718781309253478
92 92 6.71973852489892
93 93 6.720037188751452
94 94 6.72074789845859
95 95 6.721114853447318
96 96 6.722094087946726
97 97 6.7226336654669945
98 98 6.724663308912165
99 99 6.7255929888360075

